A Study in Improving BLEU Reference Coverage with Diverse Automatic Paraphrasing

We investigate a long-perceived shortcoming in the typical use of BLEU: its reliance on a single reference. Using modern neural paraphrasing techniques, we study whether automatically generating additional diverse references can provide better coverage of the space of valid translations and thereby improve its correlation with human judgments. Our experiments on the into-English language directions of the WMT19 metrics task (at both the system and sentence level) show that using paraphrased references does generally improve BLEU, and when it does, the more diverse the better. However, we also show that better results could be achieved if those paraphrases were to specifically target the parts of the space most relevant to the MT outputs being evaluated. Moreover, the gains remain slight even when human paraphrases are used, suggesting inherent limitations to BLEU's capacity to correctly exploit multiple references. Surprisingly, we also find that adequacy appears to be less important, as shown by the high results of a strong sampling approach, which even beats human paraphrases when used with sentence-level BLEU.

==> figures/manual-paraphrase-examples.tex <==
\begin{figure*}[!ht]
    \centering\small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{L{2.4cm}L{2.75cm}L{2.55cm}L{2.1cm}L{2.75cm}L{2.1cm}}
    \toprule
    Reference & Paraphrase 1 & Paraphrase 2 & Paraphrase 3 & Paraphrase 4 & Paraphrase 5 \\
    \midrule
      Yet she does not offer any proof in the clip. & However she does not give any evidence in the video. &	However, she does not offer any evidence in the clip. & But in the clip she doesn't offer any proof. & But the clip does not show her providing any evidence. &  However, she gives no proof in the clip. \\
    \midrule
    Now they have come to an agreement.  & They have now come to an agreement. & An agreement has now been made. & They have reached an agreement. &  After all this time, they have come up with an agreement. & They have finally come to a solution.\\
    \midrule
    From A-Z, update at 04/05/2018 at 11:11 & From A-Z, updated on 11:11 on 04/05/2018. & From A to Z - updated on 04.05.2018 at 11:11 & From A-Z updated on 4th May 2018. & From A to Z, updated on 04/05/2018 at 11:11 & From A to Z, updated at 11:11 on May 4, 2018 \\
    \bottomrule
    \end{tabular}}
    \caption{Examples of manually created paraphrases from the WMT19 DE-EN test set}
    \label{fig:manual-paraphrases}
\end{figure*}

==> sections/manual-analysis.tex <==
\todo[inline]{Important things to be looked at here}
\emph{The results are surprising: Can we work out why these things occur?}

\begin{itemize}
    \item Why does adding references degrade the correlation for some languages?
    \item Why do structurally diverse references not produce better correlations?
    \item Is this a problem with the (i)~paraphrases, (ii)~the way BLEU functions or (iii)~the DA assessments...
\end{itemize}

Not so manual but...



==> sections/related-work-bleu.tex <==


\bleu \citep{papineni-etal-2002-bleu} is the most used automatic
evaluation metric in MT.  It is a document-level metric that works by
accumulating over all sentences counts between the overlap between
sequences of tokens ($n$-grams) in a machine translated text and
human-produced reference translation.
%
A modified form of $n$-gram precision, it is calculated by averaging
$n$-gram precisions ($p_n$, $n = 1..4$) and multiplying by a brevity
penalty (BP) used to penalise overly short translations:
\begin{align}
\text{\bleu} &= \text{BP} \cdot \exp\left(\sum_{n=1}^N w_n \log p_n \right)
\\
\text{BP} &= 
\begin{cases}
    1 \quad\quad\quad\text{ if } c > r\\
    e^{1-r/c} \quad\text{ if } c \leq r 
\end{cases} \\
p_n &= \dfrac{\sum_{h\in H} \sum_{\text{ngram}\in h} \#_{\text{clip}}\left(\textit{ngram}\right)}{\sum_{h'\in H} \sum_{\text{ngram'}\in h'} \#\left(\textit{ngram'}\right)},
\label{eq:ngramprecisions}
\end{align}
with $c$ and $r$ the lengths of the hypothesis and reference sets
respectively, $H$ is the set of hypothesis translations,
$\#\left(\textit{ngram}\right)$ the number of times $\textit{ngram}$
appears in the hypothesis, and \#$_{\text{clip}}(\textit{ngram})$ is
the same but clipped to the maximum number of times it appears in any
one reference.

The metric is more reliable when calculated over a large test set, and
so \bleu scores are traditionally calculated on the corpus-level. The
sentence-level variant requires a smoothing strategy to counteract the
effect of 0 $n$-gram precisions, which are more probable with shorter
texts.

\bleu has received fervent criticism
\citep{callison-burch-etal-2006-evaluating} mainly due to its lack of
flexibility to surface form variation. Take for instance the three MT
outputs in Example~(\ref{ex:multiple-translations}), all valid but
different from the reference. The number of matching tokens (indicated
in bold) vary for each output, MT$_3$ having no tokens in common with
the reference, despite being a valid translation.

 

==> tables/bleu.tex <==
\begin{tabular}{l|rr}
\toprule
& \textsc{Online-B} & all \\
\midrule
none & 37.1 & 28.9 \\
\midrule
\beam & 46.4 & 37.2 \\
\random  & 43.8 & 34.9 \\
\sampled & 49.3 & 40.1 \\ 
\midrule
\laser & 46.8 & 37.7 \\
\treelstmplain  & 47.4 & 38.2 \\
constraints & 55.2 & 46.1 \\
\midrule 
human & 55.5 & 48.9 \\
\bottomrule 
\end{tabular}
\caption{Mean BLEU scores across all language pairs with five references from different paraphrase models.}
\label{table:bleu}

==> tables/improvements-vs-degradations.tex <==
\iffalse
\begin{table}[!ht]
    \centering\small
    \begin{tabular}{lrr}
    \toprule
    & \multicolumn{2}{c}{\# relative ranking assessments} \\
    Lang. dir. & degraded & improved \\
    \midrule
    cs-en & \textbf{574} & 566 \\
    de-en & 5115 & \textbf{6365} \\
    et-en & 4894 & \textbf{5266} \\
    fi-en & 1636 & \textbf{1759} \\
    ru-en & 912 & \textbf{1022} \\
    tr-en & 1007 & \textbf{1073} \\
    zh-en & \textbf{3259} & 3171 \\
    \bottomrule
    \end{tabular}
    \caption{Number of comparisons for which the relative ranking decision is reversed between the sacreBLEU-sentBLEU baseline and the \textsc{treelstm-plain (+20)} system. WMT18}
    \label{tab:seg-level-improved-worsened}
\end{table}
\fi

\begin{table*}[!ht]
    \centering\small
     \resizebox{\textwidth}{!}{
    \begin{tabular}{llrrrrrrrrrrrrrr}
    \toprule
    & & \multicolumn{2}{c}{cs-en} & \multicolumn{2}{c}{de-en} & \multicolumn{2}{c}{et-en} & \multicolumn{2}{c}{fi-en} & \multicolumn{2}{c}{ru-en} & \multicolumn{2}{c}{tr-en} & \multicolumn{2}{c}{zh-en} \\
    Approach & Method  & - & + & - & + & - & + & - & + & - & + & - & + & - & + \\
    \midrule
    \multirow{3}{*}{Baselines} 
    & beam (+5) & 8.2 & 8.0 & 4.9 & 6.4 & 6.6 & 7.5 & 7.0 & 7.5 & 6.4 & 7.3 & 8.2 & 10.1 & 6.6 & 7.1 \\
    & sampled (+5)  & 9.0 & 9.4 & 5.4 & 7.1 & 7.5 & 8.2 & 8.6 & 9.4 & 7.0 & 8.4 & 9.2 & 10.8 & 7.7 & 8.4 \\
    & random (+5) & 6.6 & 5.9 & 3.7 & 5.0 & 5.5 & 5.7 & 5.8 & 5.7 & 5.1 & 5.9 & 6.6 & 7.6 & 5.2 & 5.7 \\
    \midrule
    \multirow{3}{*}{Diversity} 
    & Laser & 8.2 & 7.7 & 4.9 & 6.4 & 6.8 & 7.2 & 7.5 & 7.9 & 6.1 & 7.3 & 8.3 & 10.2 & 6.7 & 7.2 \\
    & \treelstmsemhash & 8.5 & 8.5 & 4.7 & 6.4 & 6.6 & 7.2 & 7.2 & 7.7 & 6.5 & 8.0 & 8.3 & 10.0 & 6.4 & 7.4 \\
    & \treelstmplain & 8.3 & 8.6 & 5.1 & 6.6 & 6.8 & 7.5 & 7.7 & 8.3 & 6.9 & 7.9 & 8.5 & 10.2 & 7.1 & 7.3 \\
    \midrule
    \multirow{3}{*}{Output-specific}
    & Laser & 2.4 & 2.9 & 1.2 & 1.2 & 0.8 & 0.7 & 3.1 & 3.3 & 3.2 & 2.7 & 1.4 & 1.3 & 2.2 & 2.1 \\
    & \treelstmsemhash & 7.6 & 6.7 & 4.4 & 5.5 & 6.1 & 6.4 & 7.0 & 6.9 & 6.7 & 6.9 & 8.2 & 9.4 & 6.0 & 6.3 \\
    & \treelstmplain & 6.3 & 7.1 & 4.5 & 5.0 & 5.9 & 6.0 & 7.6 & 8.0 & 6.6 & 6.7 & 7.3 & 8.2 & 6.4 & 6.3  \\
    \multirow{3}{*}{Constrained}
    & All \\
    & Top systems \\
    \bottomrule
    \end{tabular}}
    \caption{Number of comparisons for which the relative ranking decision is reversed between the sacreBLEU-sentBLEU baseline and the \textsc{treelstm-plain (+20)} system. WMT18}
    \label{tab:seg-level-improved-worsened-wmt18}
\end{table*}

\begin{table*}[!ht]
    \centering\small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{llrlrlrlrlrlrlrl}
    \toprule
    & & \multicolumn{2}{c}{de-en} & \multicolumn{2}{c}{fi-en} & \multicolumn{2}{c}{gu-en} & \multicolumn{2}{c}{kk-en} & \multicolumn{2}{c}{lt-en} & \multicolumn{2}{c}{ru-en} & \multicolumn{2}{c}{zh-en} \\
    & & - & + & - & + & - & + & - & + & - & + & - & + & - & + \\
    \midrule
    \multirow{3}{*}{Baseline}
    & beam (+5)  & 6.5 & 6.9 & 6.9 & 8.0 & 5.9 & 6.7 & 5.9 & 6.1 & 6.9 & 8.2 & 7.1 & 7.8 & 5.7 & 5.7 \\
    & sampled (+5) & 7.3 & 7.9 & 7.6 & 8.5 & 6.5 & 7.7 & 6.4 & 7.0 & 7.4 & 9.6 & 8.0 & 9.0 & 7.3 & 7.5 \\
    & random (+5) & 4.8 & 5.3 & 5.4 & 5.9 & 4.4 & 5.0 & 4.6 & 4.7 & 5.4 & 6.7 & 5.5 & 6.1 & 4.8 & 4.9 \\
    \midrule
    \multirow{3}{*}{Diversity}
    & Laser & 6.9 & 7.1 & 7.0 & 7.9 & 6.2 & 6.7 & 5.9 & 6.2 & 7.1 & 8.5 & 7.4 & 7.9 & 6.1 & 6.1 \\
    & \treelstmsemhash & 6.7 & 7.0 & 6.9 & 7.8 & 6.3 & 6.8 & 5.6 & 6.1 & 7.0 & 8.6 & 7.3 & 8.1 & 6.1 & 6.2 \\
    & \treelstmplain & 7.0 & 7.5 & 7.2 & 8.1 & 6.1 & 7.2 & 6.2 & 6.6 & 7.2 & 8.5 & 7.7 & 8.1 & 6.5 & 6.3 \\
    \midrule
    \multirow{3}{*}{Output-specific}
    & Laser & 4.8 & 6.9 & 5.3 & 5.4 & 5.0 & 5.2 & 4.9 & 4.7 & 5.3 & 5.3 & 5.4 & 6.0 & 5.3 & 4.8 \\
    & \treelstmsemhash & 1.3 & 1.3 & 1.6 & 1.4 & 1.5 & 1.2 & 1.7 & 1.1 & 0.5 & 0.3 & 1.4 & 1.5 & 2.2 & 1.1\\
    & \treelstmplain & 1.7 & 2.8 & 2.1 & 1.8 & 1.9 & 1.8 & 2.5 & 1.7 & 0.7 & 0.7 & 2.2 & 2.3 & 2.4 & 1.8 \\
    & Parse-multi & 6.3 & 6.3 & 5.7 & 6.5 & 5.9 & 5.9 & 5.3 & 5.6 & 6.5 & 6.9 & 6.5 & 6.6 & 5.5 & 5.5 \\
    \multirow{3}{*}{Constrained}
    & All \\
    & Top systems \\
    \bottomrule
    \end{tabular}}
    \caption{Number of comparisons for which the relative ranking decision is reversed between the sacreBLEU-sentBLEU baseline and the \textsc{treelstm-plain (+20)} system. WMT19}
    \label{tab:seg-level-improved-worsened-wmt19}
\end{table*}

==> tables/paraphrase-eval/subsample-DA-adequacy.tex <==

\begin{table}[!ht]
\centering\small
\begin{tabular}{lrr|r}
\toprule
Method & adequacy & BLEU & BLEU \\
\midrule
none (ref only)   &  -   & 43.2 & 37.1 \\
\midrule
\beam             & 91.7 & 50.3 & 46.4   \\
\random           & -    & 48.1 & 43.8   \\
\sampled          & 85.0 & 51.4 & 49.3   \\
\laser            & 90.1 & 50.5 & 46.8   \\
\treelstmplain    & 88.0 & 51.1 & 47.4   \\
\midrule
constraints       & -    & 60.8 & 55.2   \\
\midrule
Human             & \textbf{95.2} & 53.2 & 55.5 \\
\bottomrule
\end{tabular}
\caption{Direct assessment scores for the first 100 sentences of the de--en test set, followed by BLEU scores of the \textsc{Online-B} system on the same data (column 2) and averaged over all sentences of all languages (column 3).}
\label{tab:subsample-DA-adequacy}
\end{table}

==> tables/parbleu-corr/wmt18-seg-normalised.tex <==
%\resizebox{\textwidth}{!}{
\small\centering
\begin{tabular}{lllllllll}
\toprule
&  & cs-en & de-en & et-en & fi-en & ru-en & tr-en & zh-en \\
Approach & Method   & \multicolumn{1}{l}{(5,110)} & \multicolumn{1}{c}{(77,811)} & (56,721) & (15,648) & (10,404) & (8,525) & (33,357) \\
\midrule

Baseline & sentence\bleu & 0.225 & 0.411 & 0.284 & 0.156 & 0.222 & 0.126 & 0.172 \\

\midrule
\multirow{3}{*}{\pbox{1.5cm}{Paraphrase baselines (+5)}}
& \beam & 0.223 & 0.443 & 0.301 & 0.162 & 0.242 & 0.164 & 0.179 \\
& \random & 0.216 & 0.437 & 0.290 & 0.155 & 0.238 & 0.145 & 0.181 \\
& \sampled \\
\midrule
\multirow{3}{*}{\pbox{1.3cm}{Diversity (+1)}} 
& \laser & 0.225 & 0.440 & 0.290 & 0.159 & 0.243 & 0.144 & 0.185 \\
& \treelstmsemhash & 0.223 & 0.434 & 0.288 & 0.162 & 0.238 & 0.149 & 0.185 \\
& \treelstmplain & 0.223 & 0.438 & 0.296 & 0.164 & 0.248 & 0.140 & 0.179 \\

\midrule
\multirow{3}{*}{\pbox{1.3cm}{Diversity (+5)}} 
& \laser & 0.214 & 0.441 & 0.292 & 0.164 & 0.245 & 0.163 & 0.182 \\
& \treelstmsemhash & 0.225 & 0.445 & 0.296 & 0.166 & 0.252 & 0.158 & 0.191 \\
& \treelstmplain & 0.232 & 0.440 & 0.297 & 0.168 & 0.242 & 0.159 & 0.175 \\

\midrule
\multirow{2}{*}{\pbox{1.3cm}{Output-specific (+1)}}
& \laser & 0.224 & 0.430 & 0.290 & 0.154 & 0.232 & 0.149 & 0.178 \\
& \treelstmsemhash & 0.236 & 0.433 & 0.290 & 0.155 & 0.225 & 0.151 & 0.176 \\
& \treelstmplain & 0.215 & 0.437 & 0.298 & 0.151 & 0.238 & 0.145 & 0.176 \\

\midrule
& \tiny WMT-18 best  &  \tiny\textbf{0.35}*** & \tiny\textbf{0.50}*** & \tiny\textbf{0.37}*** & \tiny\textbf{0.27}*** & \tiny\textbf{0.31}*** & \tiny\textbf{0.26}*** & \tiny\textbf{0.22}**  \\
 & & \tiny \textsc{RUSE} & \tiny \textsc{RUSE} & \tiny \textsc{RUSE} & \tiny \textsc{RUSE} & \tiny \textsc{RUSE} & \tiny \textsc{RUSE} & \tiny \textsc{RUSE} \\
\bottomrule
\end{tabular}%}

==> tables/parbleu-corr/wmt18-sys-normalised.tex <==
\scalebox{1}{
\centering\small
\begin{tabular}{lllllllll}
\toprule
&& cs-en & de-en & et-en & fi-en & ru-en & tr-en & zh-en \\
Approach & Method   & (5) & (16) & (14) & (9) & (8) & (5) & (14) \\
\midrule

Baseline & \bleu & 0.955 & 0.967 & 0.987 & 0.962 & 0.966 & -0.944 & 0.985 \\

\midrule
\multirow{3}{*}{\pbox{1.5cm}{Paraphrase baselines (+5)}}
& \beam & 0.966 & 0.973 & 0.995** & 0.957 & 0.965 & -0.357* & 0.989 \\
& \random & 0.968 & 0.972 & 0.994** & 0.958 & 0.966 & -0.810 & 0.989 \\
& \sampled \\
\midrule
\multirow{3}{*}{\pbox{1.3cm}{Diversity (+1)}} 
& \laser & 0.967 & 0.971 & 0.993** & 0.956 & 0.966 & -0.708* & 0.989 \\
& \treelstmsemhash & 0.963 & 0.971 & 0.993** & 0.958 & 0.968 & -0.835 & 0.989 \\
& \treelstmplain & 0.964 & 0.970 & 0.994*** & 0.957 & 0.966 & -0.851* & 0.990 \\

\midrule
\multirow{3}{*}{\pbox{1.3cm}{Diversity (+5)}} 
& \laser & 0.969 & 0.972 & 0.995** & 0.953 & 0.966 & -0.021* & 0.987 \\
& \treelstmsemhash & 0.964 & 0.973 & 0.995** & 0.954 & 0.968 & -0.618 & 0.988 \\
& \treelstmplain & 0.964 & 0.973 & 0.996** & 0.956 & 0.965 & -0.273 & 0.988 \\

\midrule
\multirow{2}{*}{\pbox{1.3cm}{Output-specific (+1)}}
& \laser & 0.958 & 0.971 & 0.993** & 0.955 & 0.966 & -0.737 & 0.988 \\
& \treelstmsemhash & 0.955 & 0.973 & 0.995** & 0.957 & 0.965 & -0.591* & 0.989 \\
& \treelstmplain & 0.957 & 0.971 & 0.994** & 0.956 & 0.967 & -0.800 & 0.988 \\

\midrule

\multirow{2}{*}{\pbox{2.4cm}{Constraints}} & All &  \\
& Top outputs  &  \\
\midrule
& WMT-18 best  &  0.981 & \textbf{0.997}*** & 0.991 & \textbf{0.996} & \textbf{0.995}* & \textbf{0.970}* & 0.982\\

& & \tiny (\textsc{RUSE})   & \tiny (\textsc{RUSE}) & \tiny (\textsc{WER}) & \tiny (\textsc{ITER}) & \tiny (\textsc{METEOR++}) & \tiny (\textsc{NIST}) & \tiny (\textsc{CDER}) \\
    \bottomrule
    \end{tabular}}





==> tables/parbleu-corr/wmt19-parbleu-summary-results.tex <==
\begin{subtable}{0.75\linewidth}
\centering\small
\scalebox{0.95}{
\begin{tabular}{llrrrrrrrr}
\toprule
&&& \multicolumn{3}{c}{System} && \multicolumn{3}{c}{Segment} \\
Approach & Method & \hphantom{oo} & Ave. & Min & Max & \hphantom{oo} & Ave. & Min & Max \\
\midrule
\multirow{3}{*}{\pbox{1.8cm}{Baselines (+5)}}
& \beam &&  2.18 & {-0.73} & \textbf{6.86}  &&  7.97 & {-0.16} & {13.19} \\
& \random &&  1.88 & {0.05} & \textbf{5.34}  &&  3.96 & {-0.57} & {6.98} \\
& \sampled &&  2.69 & {-0.16} & \textbf{7.78}  &&  11.95 & {-1.36} & {33.70} \\
\midrule
\multirow{2}{*}{\pbox{1.8cm}{Diversity (+1)}}
& \laser &&  1.92 & {-0.05} & \textbf{5.52}  &&  6.02 & {-0.95} & {12.32} \\
& \treelstm &&  1.94 & {-0.05} & \textbf{5.62}  &&  6.50 & {-0.59} & {11.25} \\
\midrule
\multirow{2}{*}{\pbox{1.8cm}{Diversity (+5)}}
 & \laser &&  2.25 & {-0.53} & \textbf{6.55}  &&  6.95 & {-0.73} & {13.07} \\
 & \treelstm &&  2.26 & {-0.37} & \textbf{6.60}  &&  8.05 & {-1.14} & {18.97} \\
%\midrule
%\multirow{2}{*}{\pbox{1.8cm}{Output-specific (+1)}}
%& \laser &&  1.35 & {-0.70} & \textbf{4.76}  &&  3.97 & {-0.37} & {10.52} \\
%& \treelstm &&  1.56 & {-0.89} & \textbf{4.81}  &&  5.26 & {-1.62} & {12.02} \\
\midrule
Constraints & 4-grams  && 2.83 & -0.16 & \textbf{7.15} && 9.98 & -26.35 & 63.17  \\% && -3.02 & 134.62 \\
%Constraints & 4-grams  && 1.90 & -2.36 & \textbf{7.89} && 10.75 & -16.58 & 26.75  \\% && -3.02 & 134.62 \\
\midrule
\human && & - & - & -  & & - & - & -  \\%&& 4.36 & 142.31 \\
WMT-19 best & Multiple && 9.25 & 1.02 & \textbf{24.28} && 84.84 & \textbf{19.57} & \textbf{92.98} \\
\bottomrule
\end{tabular}}
\caption{\label{tab:correl-all}Average and minimum and maximum gains over all into-English test sets}
\end{subtable}
\begin{subtable}{0.19\linewidth}
\small
\scalebox{0.95}{
\begin{tabular}{rr}
\toprule
System & Segment \\
\multicolumn{2}{c}{de--en} \\
\midrule
\textbf{4.43}   &  {82.11}  \\
\textbf{3.50}   &  {63.86}  \\
\textbf{4.93}   &  {164.21}  \\
\midrule
\textbf{3.77}   &  {85.26}  \\
\textbf{3.50}   &  {40.35}  \\
\midrule
\textbf{4.49}   &  {85.96}  \\
\textbf{4.89}   &  {29.12}  \\
% Output-specific
%\midrule
%\textbf{3.54}   &  {57.89}  \\
%\textbf{4.39}   &  {42.11}  \\
\midrule
% Constraints
\textbf{4.24} & 146.15 \\
\midrule
\textbf{5.99}   &  {140.35}  \\
 - & - \\
\bottomrule
\end{tabular}}
\caption{\label{tab:correl-500-subset}500-sample subset}
\end{subtable}














\iffalse
\begin{subtable}{0.75\linewidth}
%\resizebox{\linewidth}{!}{
\scalebox{0.95}{
\centering\small
\begin{tabular}{llrrrrrrrr}
\toprule
%         &        && \multicolumn{7}{c}{\textbf{All into-English test sets}} \\%& \multicolumn{3}{c}{\textbf{500-sample subset}} \\
         &        &&  \multicolumn{3}{c}{System} && \multicolumn{3}{c}{Segment} \\%& \\
Approach & Method & \hphantom{oo} & Ave. & Min & Max & \hphantom{oo} & Ave. & Min & Max \\%&& System & Segment \\

\midrule
\multirow{3}{*}{\pbox{1.5cm}{Baselines (+5)}}
& \beam &&  2.18 & -0.75 & \textbf{6.84}     &&  7.783 & 0.00 & 13.16    \\%&&  4.36 & 84.62 \\
& \random && 1.88 & 0.10 & \textbf{5.34}     &&  3.92 & -0.63 & 7.17    \\%&&  3.46 & 65.38 \\
& \sampled && 2.70 & -0.13 & \textbf{7.77}   &&  11.69 & -1.26 & 17.53   \\%&&  4.92 & 165.38 \\

\midrule
\multirow{2}{*}{\pbox{1.5cm}{Diversity (+1)}}
& \laser && 1.92 & 0.00 & \textbf{5.45}      && 5.71 & -0.95 & 9.96       \\%&& 3.80 & 88.46\\
%& \treelstmsemhash & 1.82 & -0.13 & \textbf{5.57}    && 6.004	0.315	11.952 \\
& \treelstmplain && 1.94 & 0.00 & \textbf{5.57} &&  6.41  & -0.63 & 10.76   \\%&& 3.46 & 42.31 \\

\midrule
\multirow{2}{*}{\pbox{1.5cm}{Diversity (+5)}}
& \laser && 2.26 & -0.50 & \textbf{6.50}      &&  6.93 & -0.63 & 13.15  \\%&& 4.47 & 88.46 \\
%& \treelstmsemhash & 2.06 & -1.25 & 6.61    && 6.826	0	13.546 \\
& \treelstmplain && 2.27 & -0.38 & \textbf{6.50}    && 7.90 & -0.95 & 11.95 \\%&& 4.92 & 30.77 \\

\midrule
\multirow{2}{*}{\pbox{1.8cm}{Output-specific (+1)}}
& \laser && 1.37 & -0.63 & \textbf{4.76}  && 3.75 & -0.32 & 6.37 \\
%& \treelstmsemhash & 1.66 & -0.63 & \textbf{5.34}  && 5.15 & -0.63 & 11.40 \\
& \treelstmplain && 1.55 & -0.88 & \textbf{4.76} && 5.06 & -1.58 & 8.57 \\

\midrule
Constraints & 4-grams  && 1.90 & -2.36 & \textbf{7.89} && 10.75 & -16.58 & 26.75  \\% && -3.02 & 134.62 \\

\midrule
Human && & - & - & -  & & - & - & -  \\%&& 4.36 & 142.31 \\
WMT-19 best & Multiple && 9.25 & 1.02 & \textbf{24.28} && 84.84 & \textbf{19.57} & \textbf{92.98} \\

\bottomrule
\end{tabular}}
\caption{\label{tab:correl-all}Average and minimum and maximum gains over all into-English test sets}
\end{subtable}
%
\begin{subtable}{0.19\linewidth}
\scalebox{0.95}{
\small
%\centering\small
\begin{tabular}{lrrrrrrr}
\toprule
%\multicolumn{3}{c}{\textbf{500-sample subset}} \\
 System & Segment \\
 \multicolumn{2}{c}{de--en} \\

\midrule
% paraphrase baselines
  4.36 & 84.62 \\
  3.46 & 65.38 \\
  4.92 & 165.38 \\

\midrule
% Diversity + 1
 3.80 & 88.46\\
 3.46 & 42.31 \\

\midrule
% Diversity + 5
 4.47 & 88.46 \\
 4.92 & 30.77 \\

\midrule
%\multirow{2}{*}{\pbox{1.8cm}{Output-specific (+1)}}
 3.46 & 57.69 \\
 4.36 & 42.31 \\

\midrule
% Constraints
 -3.02 & 134.62 \\

\midrule
% Human
4.36 & 142.31 \\
 - & - \\
\bottomrule
\end{tabular}}
\caption{\label{tab:correl-500-subset}500-sample subset}
\end{subtable}
\fi

==> tables/parmeteor-corr/parmeteor-wmt18-seglevel.tex <==

\resizebox{\textwidth}{!}{
\begin{tabular}{lllllllll}
\toprule
&  & cs-en & de-en & et-en & fi-en & ru-en & tr-en & zh-en \\
Approach & Method   & \multicolumn{1}{l}{(5,110)} & \multicolumn{1}{c}{(77,811)} & (56,721) & (15,648) & (10,404) & (8,525) & (33,357) \\
\midrule
% Results different from the official ones
Baseline & sentenceMeteor & 0.243 &  0.433 &  0.309 &  0.175 &  0.231 &  0.147 &  0.183 \\
\midrule
\multirow{3}{*}{\pbox{1.5cm}{Paraphrase baselines (+5)}}
& \beam & 0.254 &  0.460 &  0.319 &  0.191 &  0.253 &  0.183 &  0.198 \\
& \random   &  0.241 &  0.450 &  0.312 &  0.192 &  0.253 &  0.168 &  0.189 \\
& \sampled  & \\

\midrule
\multirow{3}{*}{\pbox{1.5cm}{Diversity (+1)}} 
& \laser & 0.251 &  0.449 &  0.309 &  0.185 &  0.242 &  0.163 &  0.192 \\
& \textsc{treelstm-semhash} & 0.254 &  0.447 &  0.310 &  0.193 &  0.245 &  0.167 &  0.194 \\
& \textsc{treelstm-plain} & 0.258 &  0.449 &  0.314 &  0.198 &  0.245 &  0.171 &  0.186 \\

\midrule
\multirow{3}{*}{\pbox{1.5cm}{Diversity (+5)}} 
& \laser & 0.248 &  0.457 &  0.310 &  0.198 &  0.255 &  0.169 &  0.195\\
& \textsc{treelstm-semhash} & 0.263 &  0.455 &  0.313 &  0.200 &  0.253 &  0.172 &  0.197 \\
& \textsc{treelstm-plain} & 0.247 &  0.454 &  0.317 &  0.212 &  0.249 &  0.180 &  0.186  \\


\midrule
\multirow{2}{*}{\pbox{1.5cm}{Output-specific (+1)} }
& \laser & 0.233 &  0.444 &  0.314 &  0.188 &  0.248 &  0.159 &  0.180 \\
& \textsc{treelstm-semhash} & 0.249 &  0.447 &  0.316 &  0.188 &  0.236 &  0.162 &  0.190 \\
& \textsc{treelstm-plain} & 0.255 &  0.452 &  0.309 &  0.196 &  0.242 &  0.154 &  0.181 \\

\midrule
& \tiny WMT-18 best  &  \tiny\textbf{0.35}*** & \tiny\textbf{0.50}*** & \tiny\textbf{0.37}*** & \tiny\textbf{0.27}*** & \tiny\textbf{0.31}*** & \tiny\textbf{0.26}*** & \tiny\textbf{0.22}**  \\
 & & \tiny \textsc{RUSE} & \tiny \textsc{RUSE} & \tiny \textsc{RUSE} & \tiny \textsc{RUSE} & \tiny \textsc{RUSE} & \tiny \textsc{RUSE} & \tiny \textsc{RUSE} \\
\bottomrule
\end{tabular}}



==> tables/parmeteor-corr/parmeteor-wmt18-syslevel.tex <==

\centering\small
\scalebox{1}{
\begin{tabular}{lllllllll}
\toprule
        && cs-en & de-en & et-en & fi-en & ru-en & tr-en & zh-en \\
    Approach & Method   & (5) & (16) & (14) & (9) & (8) & (5) & (14) \\
    \midrule
    
% Results different from the official ones
Baseline & Meteor & 0.977 & 0.989 & 0.987 & 0.995 & 0.979 & -0.859 & 0.980 \\
\midrule
\multirow{3}{*}{\pbox{1.5cm}{Paraphrase baselines (+5)}}
& \beam & 0.986 & 0.992 & 0.991* & 0.997 & 0.979 & -0.688 & 0.987* \\
& \random & 0.983 & 0.991* & 0.990 & 0.997* & 0.981 & -0.782 & 0.985* \\
& \sampled & \\

\midrule
\multirow{3}{*}{\pbox{1.5cm}{Diversity (+1)}} 
& \laser & 0.981 & 0.991* & 0.991* & 0.997* & 0.979 & -0.753 & 0.986** \\
& \textsc{treelstm-semhash} & 0.982 & 0.992* & 0.991* & 0.997 & 0.981 & -0.777 & 0.986* \\
& \textsc{treelstm-plain} & 0.983 & 0.991 & 0.990 & 0.997* & 0.979 & -0.760 & 0.987**  \\

\midrule
\multirow{3}{*}{\pbox{1.5cm}{Diversity (+5)}} 
& \laser & 0.983 & 0.992 & 0.992* & 0.997 & 0.979 & -0.562* & 0.988* \\
& \textsc{treelstm-semhash} & 0.982 & 0.992* & 0.992* & 0.997 & 0.981 & -0.713 & 0.988*  \\
& \textsc{treelstm-plain} & 0.984 & 0.992* & 0.991 & 0.997 & 0.979 & -0.597 & 0.988** \\


\midrule
\multirow{2}{*}{\pbox{1.5cm}{Output-specific (+1)} }
& \laser & 0.977 & 0.991 & 0.991* & 0.997 & 0.980 & -0.724 & 0.985* \\
& \textsc{treelstm-semhash} & 0.978 & 0.992* & 0.991 & 0.997* & 0.980 & -0.644* & 0.986* \\
& \textsc{treelstm-plain} & 0.978 & 0.992* & 0.991* & 0.997 & 0.980 & -0.707* & 0.987* \\

& WMT-18 best  &  0.981 & \textbf{0.997}*** & 0.991 & \textbf{0.996} & \textbf{0.995}* & \textbf{0.970}* & 0.982\\
& & \tiny (\textsc{RUSE})   & \tiny (\textsc{RUSE}) & \tiny (\textsc{WER}) & \tiny (\textsc{ITER}) & \tiny (\textsc{METEOR++}) & \tiny (\textsc{NIST}) & \tiny (\textsc{CDER}) \\
    \bottomrule
\end{tabular}}


